Efficient training sets for surrogate models of tokamak turbulence with Active Deep Ensembles

Model-based plasma scenario development lies at the heart of the design and operation of future fusion powerplants. Including turbulent transport in integrated models is essential for delivering a successful roadmap towards operation of ITER and the design of DEMO-class devices. Given the highly iterative nature of integrated models, fast machine-learning-based surrogates of turbulent transport are fundamental to fulfil the pressing need for faster simulations opening up pulse design, optimization, and flight simulator applications. A significant bottleneck is the generation of suitably large training datasets covering a large volume in parameter space, which can be prohibitively expensive to obtain for higher fidelity codes. In this work, we propose ADEPT (Active Deep Ensembles for Plasma Turbulence), a physics-informed, two-stage Active Learning strategy to ease this challenge. Active Learning queries a given model by means of an acquisition function that identifies regions where additional data would improve the surrogate model. We provide a benchmark study using available data from the literature for the QuaLiKiz quasilinear transport model. We demonstrate quantitatively that the physics-informed nature of the proposed workflow reduces the need to perform simulations in stable regions of the parameter space, resulting in significantly improved data efficiency. We show an up to a factor of 20 reduction in training dataset size needed to achieve the same performance as random sampling. We then validate the surrogates on multichannel integrated modelling of ITG-dominated JET scenarios and demonstrate that they recover the performance of QuaLiKiz to better than 10\%. This matches the performance obtained in previous work, but with two orders of magnitude fewer training data points.

==> junk.tex <==

\begin{comment}

\subsubsection{Why does the classifier perform better than random?}
\begin{figure}
    \centering
    \includegraphics[width=0.9 \textwidth]{plots/0_allfluxes.pdf}
    \caption{Left: 2D UMAP \cite{mcinnes2020umap} projection of the JetExp dataset. Orange and cyan dots represent the stable and unstable regions in the test set. Blue stars (red diamonds) indicate the candidates selected and the presence (absence) of growing modes. Right: Normalised histograms of the regressor uncertainty of candidates selected by the classifier to be stable. The vertical dashed line indicates the uncertainty associated to the least uncertain point of the sample selected for acquisition. As the classifier is not 100\% accurate, both stable (red) and unstable (blue) regions are considered by the regressor. Therefore, some of the stable points are also selected for acquisition.  }
    \label{fig:UMAP}
\end{figure}
The first interesting feature of the two-stage framework is that the classifier performance improves with the size of the training set better than random while not explicitly featuring in the acquisition function. This is a result of the interplay between the classifier and the regressor networks. Since the classifier is not perfect, therefore some inputs are classified as unstable while in reality they are not. Thus, as the right panel of Figure~\ref{fig:UMAP} shows, the uncertainty distribution for candidate points to be evaluated by the acquisition function contains inputs resulting in both stable and unstable modes. Some of the stable inputs are therefore queried and are added to the training set of the classifier. Hence, the classifier is also trained on a biased region of the input space. This can be observed in the left hand side of Figure \ref{fig:UMAP} which shows the input parameter space in projected on a 2D domain using UMAP \cite{mcinnes2020umap}, a popular dimensionality reduction technique. 

In summary, the two-stage physics-informed nature of the AL pipeline naturally results in an exchange of information between the classifier and the regressor NNs, and thus efficient learning of both the critical gradient threshold and the values of the fluxes.
\end{comment}
%\subsection{Where does uncertainty-driven AL benefit surrogates the most?}

   
%\textbf{however it's easy to predict zeros!! Especially when 75% of the data is zero, what has the model actually learned? show plot with non physics informed tested on non zeros} 

\begin{comment}
\subsubsection{Beware underparametrising NNs for AL tasks}
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{plots/doubledescent.pdf}
    \caption{The "double descent" behaviour in shallow Neural Networks. There is a regime  where more training data hurts performance.}
    \label{fig:doubledescent}
\end{figure}
Conventional wisdom from statistics is that larger statistical models suffer from significant overfitting unless explicitly and, sometimes, strongly regularised. Recent work \cite{nakkiran2019deep} has shown that as the size of a NN increases, performance on the test set first improves (under-parametrised regime), then it deteriorates when the number of training samples are similar to the number of the network parameters (interpolation threshold) and finally it improves once again and exceeds the performance of the under-parametrised regime for large models (interpolating regime). This behaviour has been named \emph{double descent}.


A consequence of the double descent phenomenon is that, at fixed model size, there is a critical regime where more data hurts performance. This is crucial in Active Learning applications, where the training dataset size increases during subsequent acquisition cycles for a fixed NN architecture. Figure \ref{fig:doubledescent} shows this behaviour in action for a 2-layer Deep Ensemble regressing to $q_{i,ITG}$ embedded in the AL pipeline. We recommend that future studies adopting AL for Fusion use cases adopt suitably large NNs to counteract the double descent phenomenon.


%Therefore, for a fixed NN architecture with a given number of parameters, an small network trained on a very small dataset can be considered in the underparametrised regime. However, as the acquisition of training data proceeds further, the NN will be pushed towards the interpolation threshold, and therefore the performance of the NN will become \emph{worse} with more data. Figure \textbf{todo} shows this behaviour in action for a 2-layer Deep Ensemble composed of five members. We also confirm that increasing the size of the NN over the interpolation threshold results in smoothly declining training curves and recommend that future studies adopting AL for Fusion use cases adopt suitably large NNs.
\end{comment}



\begin{comment}
    

\begin{itemize}
    \item show UMAP embedding of test data, color coded by classification and regressor, uncertainty, inputs and flux outputs
    \item experiment with RHO-loss  from Gal's paper as an upper limit to performance
\end{itemize}
\end{comment}



\begin{comment}

\subsubsection{Maximum informativeness and uncertainty sampling}
The goal of Active Learning is to obtain a machine learning predictive model by identify training points that are more efficient than random selection. Space-filling methods, such as Latin Hypercube Sampling (LHS,\cite{McKay1979}), have been shown to improve upon random selection, however the LHS algorithm samples the input space just once, and therefore does not account for potential redundancies in the information provided by different inputs. A more efficient query strategy consists in maximising the informativeness of the training sample as a whole. Given a random variable $X$ with probability distribution $p_X$ and an observation $x$, information is defined mathematically following \cite{shannonMathematicalTheoryCommunication1948} as:
\begin{equation}
    I_X = -\log{p_X(x)}.
    \label{eq:1}
\end{equation}
The definition above maximises the degree of ``surprise'' of a given observation $x$. A probability of 1 yields no information, and small probabilities yield large information.
A useful related quantity is the entropy $\mathcal{H}$, defined as the average expectation of information, which quantifies the amount of uncertainty in a distribution,
\begin{equation}
    \mathcal{H} = - \sum_{i=1}^N p_X(x_i)\log{p_X(x_i)}.
    \label{eq:2}
\end{equation}
An equivalent integral formulation applies for continuous distributions. For example, given a hypotetical training set $D_{train}=\{ x_{train,i},y_{train,i} \}_{i=1}^N $ and a learner $f$ equipped with a covariance matrix $\textbf{K}$ (such as a Gaussian Process or, indeed, a NN \cite{lee2017deep}), the entropy of a subset of size $n<N$ can be expressed in terms of the determinant of $\textbf{K}$ as
\begin{equation}
    \mathcal{H}(Y_{n}) = \frac{1}{2}\log{\bigl ( (2\pi e)^{n} det(\textbf{K}))\bigr ).
    \label{eq:3}
\end{equation}

Maximum entropy sampling \cite{MaxEntropy} is therefore a natural choice to identify the most informative points to train a learner. To generate the most informative dataset of size N subject to a fixed computational budget, the optimisation problem below can be solved
\begin{equation}
    x_{train}= \underset{x \in \mathcal{U}}{arg\ max} \ \mathcal{H}
    \label{eq:4}
\end{equation}
where $\mathcal{U}$ is the unlabelled pool of inputs. Unfortunately, this is intractable computationally \cite{Maxentropy_NP_Hard}. Actively Learning \emph{sequentially} the most informative training data constitutes a more  computationally affordable strategy, albeit suboptimal.
\end{comment}

